Inequality of Opportunity and Income Redistribution

Opportunities, such as access to education or family background, shape income inequality by influencing the chances of economic success. Unequal opportunities create uncertainty about whether success is merit- or luck-based. We examine how uncertainty impacts preferences for redistribution, comparing it to more transparent forms of luck. Using a U.S.-representative sample, we elicit redistribution decisions in two environments: when workers' earnings are influenced by luck directly ("lucky outcomes") or indirectly ("lucky opportunities"). Spectators redistribute less and are less sensitive to differences in luck under opportunities. Inferential challenges drive this gap, which implies that individuals are less meritocratic than previous findings suggest.

==> tables/pred-luck-connections.tex <==
Success is about luck ($-$)&&$-$0.048&&$-$0.113&\sym{*}&0.065&\\
&&(0.042&)&(0.054&)&(0.068&)\\


==> tables/pred-r2.tex <==
R$-$squared&&0.005&&0.016&&0.011&\\


==> tables/redist-het-better-life.tex <==
Hard work brings a better life&&$-$0.063&\sym{**}&$-$0.002&&$-$0.046&&0.002&\\
&&(0.022&)&(0.009&)&(0.026&)&(0.008&)\\


==> tables/redist-het-black.tex <==
Black&&0.038&&$-$0.017&&$-$0.061&&0.027&\\
&&(0.033&)&(0.012&)&(0.049&)&(0.017&)\\


==> tables/redist-het-high-numeracy.tex <==
High numeracy&&$-$0.011&&0.042&\sym{***}&0.034&&0.034&\sym{***}\\
&&(0.025&)&(0.009&)&(0.026&)&(0.009&)\\


==> tables/redist-het-issues-democrat.tex <==
Tend to side with democrats&&0.004&&$-$0.006&&0.062&\sym{*}&$-$0.011&\\
&&(0.021&)&(0.009&)&(0.025&)&(0.007&)\\


==> tables/redist-het-low-income.tex <==
HH income below 100k&&0.050&\sym{*}&$-$0.013&&0.046&&$-$0.004&\\
&&(0.024&)&(0.009&)&(0.026&)&(0.007&)\\


==> tables/redist-het-low-numeracy.tex <==
Low numeracy&&0.011&&$-$0.042&\sym{***}&$-$0.034&&$-$0.034&\sym{***}\\
&&(0.025&)&(0.009&)&(0.026&)&(0.009&)\\


==> tables/redist-het-luck-connections.tex <==
Success is about luck&&0.021&&0.005&&0.037&&$-$0.005&\\
&&(0.026&)&(0.010&)&(0.028&)&(0.009&)\\


==> tables/redist-het-male.tex <==
Male&&$-$0.045&\sym{*}&0.015&&$-$0.054&\sym{*}&0.001&\\
&&(0.020&)&(0.009&)&(0.025&)&(0.007&)\\


==> tables/redist-het-nocollege.tex <==
Less than college&&0.015&&$-$0.014&&$-$0.023&&$-$0.011&\\
&&(0.022&)&(0.009&)&(0.027&)&(0.008&)\\


==> tables/redist-het-old.tex <==
Over 50$-$years old&&0.017&&$-$0.007&&0.040&&$-$0.003&\\
&&(0.021&)&(0.009&)&(0.025&)&(0.007&)\\


==> tables/redist-het-redistribute-regardless.tex <==
Gov't eliminate income differences&&0.035&&$-$0.013&&0.042&&$-$0.014&\\
&&(0.040&)&(0.014&)&(0.037&)&(0.011&)\\


==> tables/redist-het-retired.tex <==
Retired&&$-$0.000&&0.024&&0.039&&$-$0.003&\\
&&(0.027&)&(0.013&)&(0.033&)&(0.010&)\\


==> tables/redist-het-working-ft.tex <==
Works full$-$time&&$-$0.034&&$-$0.000&&$-$0.035&&0.004&\\
&&(0.021&)&(0.010&)&(0.025&)&(0.007&)\\


==> tables/spectator-summ-pol.tex <==
Democrat &0.39 & &0.40 &0.45 &0.40 & &0.38 &0.36 &0.37 \\
Republican &0.32 & &0.29 &0.37 &0.32 & &0.29 &0.34 &0.32 \\
Influence of hard work is fair &0.88 & &0.86 &0.90 &0.90 & &0.84 &0.91 &0.85 \\
Influence of talent is fair &0.84 & &0.81 &0.86 &0.84 & &0.79 &0.89 &0.86 \\
Influence of luck is fair &0.35 & &0.32 &0.39 &0.32 & &0.31 &0.40 &0.35 \\
Influence of connections are fair &0.23 & &0.21 &0.21 &0.23 & &0.22 &0.24 &0.24 \\

